A Double Auction Mechanism for Mobile Crowd Sensing with Data Reuse

Mobile Crowd Sensing (MCS) is a new paradigm of sensing, which can achieve a flexible and scalable sensing coverage with a low deployment cost, by employing mobile users/devices to perform sensing tasks. In this work, we propose a novel MCS framework with data reuse, where multiple tasks with common data requirement can share (reuse) the common data with each other through an MCS platform. We study the optimal assignment of mobile users and tasks (with data reuse) systematically, under both information symmetry and asymmetry, depending on whether the user cost and the task valuation are public information. In the former case, we formulate the assignment problem as a generalized Knapsack problem and solve the problem by using classic algorithms. In the latter case, we propose a truthful and optimal double auction mechanism, built upon the above Knapsack assignment problem, to elicit the private information of both users and tasks and meanwhile achieve the same optimal assignment as under information symmetry. Simulation results show by allowing data reuse among tasks, the social welfare can be increased up to 100~380%, comparing with those without data reuse. We further show that the proposed double auction is not budget balance for the auctioneer, mainly due to the data reuse among tasks. To this end, we further introduce a reserve price into the double auction (for each data item) to achieve a desired tradeoff between the budget balance and the social efficiency.

==> Section4-Randomized.tex <==
%!TEX root = Data_Reuse_MCS.tex



\subsection{Information Asymmetry}



%Inspired by the randomized auction in \cite{ra,RAuction}, we now propose a low-complexity truthful randomized auction mechanism, which operates in polynomial time.
%It is important to note that due to the two-sided structure, our auction is different from the traditional single-sided auctions \cite{ra,RAuction}.  %{(defined in Section \ref{sec:ram})}.

%\com{hard to understand. we should emphasize it as the approach's approximation from VCG}

Now we propose a low-complexity truthful randomized auction mechanism for solving Problem P1 in polynomial time.
We start from the linear programming relaxation of Problem P1, obtaining an associated linear programming Problem P2 \emph{in the fractional domain}, from which we further derive the fractional VCG auction (which may not be implementable in practice).
Then, through proper decompositions, we transform the fractional VCG auction to the two-sided randomized auction (which is implementable).

%Key idea: Integer Programming --$>$ Linear Programming Relaxation --$>$
%Fractional Truthful Mechanism --$>$ Randomized Truthful Mechanism

\subsubsection{\textbf{Linear Programming Relaxation}}

We first relax Problem P1 to the fractional domain (i.e., every binary variable in the set $\{0, 1\}$ is relaxed to the interval $[0,1]$), and denote the associated linear programming problem as Problem P2.
%\com{See my comment of Problem P1. }
% \begin{equation}\label{eq:p2}
% \begin{aligned}
% \mbox{P2:} & & \max_{\x , \boldsymbol{y}, \z } & ~~~ V(\z ) - C(\x )
% \\
% & & \mbox{s.t.} & ~~~  \eqref{eq:zj}\mbox{--}\eqref{eq:yk}, \quad \forall i \in \I, j \in \J, k \in \D;
% \\
% & & \mbox{var.} & ~~~  x_i(\S) \in [0, 1],\quad \forall \S\in\S_i, i \in \I ;
% \\
% & & & ~~~   z_j \in [0, 1],\quad \forall j \in \J ;\\
% & &  & ~~~ y_k \in [0, 1],\quad \forall   k \in \D.
% \end{aligned}
% \end{equation}
Note that Problem P2 can be solved to its optimality  in polynomial time as it is a standard linear programming\cite{lp}.
We refer to the solution to Problem P2 as the \emph{fractional optimal solution}, denoted by
$\{\x ^\ast, \boldsymbol{y}^\ast, \z ^\ast\}$ or $\{\x ^\ast (\boldsymbol{c},\v), \boldsymbol{y}^\ast(\boldsymbol{c},\v), \z ^\ast(\boldsymbol{c},\v)\}$.
It is notable  that the solution to Problem P2 provides an upper-bound for that to Problem P1, and the gap between them is  called  the \emph{integrality gap} \cite{lp}.
% \com{Give a reference. }
Intuitively, a fractional solution can be viewed as \emph{the fraction of the time} that users are scheduled or tasks are selected.

Next, we propose the fractional VCG auction $\mech^\ast$, where the allocation rule aims to maximize the social welfare (defined on user bids $\b $ and task bids $\bv $)  \emph{in the fractional domain},
and the payment rule aims to pay each scheduled user its social benefit and charge each selected task its social damage. The detailed mechanism is similar to $\mech^o$, except that we replace the integer solution $\{\x ^o(\b,\bv ),\z ^o(\b,\bv )\}$ by the fractional optimal solution $\{\x ^\ast(\b,\bv ),\z ^\ast(\b,\bv )\}$, and solving Problem P2 rather than Problem P1 when deciding the payments.
%Formally,

%\com{Modify Mechanism 2 similar as Mechanism 1. }

% \begin{mechanism}[Fractional Two-sided VCG Auction -- $\mech^\ast$]\label{mech:2}
% ~
% \begin{itemize}
% \item
% Allocation Rule $\{\x  (\b,\bv ),\z   (\b,\bv )\}$:
% $$
% \x (\b,\bv ) = \x ^\ast(\b,\bv ) \mbox{~~and~~}
% \z  (\b ,\bv)= \z ^\ast(\b,\bv ),
% $$
% where $\{\x ^\ast(\b,\bv ), \z ^\ast(\b,\bv )\}$ is the solution to Problem P2 by replacing the real sensing cost $\boldsymbol{c}$ with the reported cost $\b $ before solving Problem P2;
% \item
% Payment Rule $\p  (\b,\bv )$:
% $$
% \p   (\b,\bv) = \p^\ast  (\b,\bv) \eq (p_i^\ast (\b,\bv))_{i\in\I},
% $$
% where
% $$ p_i^\ast  (\b,\bv) \eq
%  \sum_{j\in \J}  v_j \cdot z_j^\ast (\b )
% - \sum_{n \in \I \setminus \{i\}} \sum_{\S \subseteq \S_n}  b_n (\S) \cdot x_n^\ast (\S)  - W^\ast_{-i} ,
% $$
% and $W^\ast_{-i}  $ is the maximum social welfare (defined on $\b $) excluding user $i$'s bid in the fractional domain.
% \end{itemize}
% \end{mechanism}

%Similarly, we summarize the properties of $\mech^\ast$ as follows.
%we can write the fractional VCG auction as $ \mech^\ast \eq \{\x^\ast (\cdot), \z^\ast(\cdot); \p^\ast(\cdot)\} $ or $ \{\x^\ast (\b), \z^\ast(\b); \p^\ast(\b)\} $. We can also show that the fractional VCG auction $\mech^\ast$ is truthful by \cite{vcg}, hence $\b  = \boldsymbol{c}$. This implies that it is efficient (i.e., maximizing the social welfare) in the fractional domain.

% \com{combine close key propositions. Similarly, Prop. 1,2}

%\com{See my comment of Propositions 1 and 2. Combine these two propositions into one and cite the reference (as this is a standard VCG auction). }

\begin{proposition} %[Truthfulness and Efficiency]
The fractional VCG auction $\mech^\ast$ is individually rational, incentive compatible (truthful), and maximizes the social welfare in the fractional domain.
\end{proposition}

%The proof is also standard and can be referred to \cite{vcg}.
Note that the optimal solution to Problem P2 (or the outcome of $\mech^\ast$) may \emph{not} be feasible to   Problem P1.
This implies that \emph{the fractional VCG auction $\mech^\ast$ may not be implementable}.
%\footnote{An artificial example is a system with 3 data items $\D=\{1,2,3\}$, 3 users $\I = \{1,2,3\}$ with sensing capabilities $\S_1=\{1,2\}$, $\S_2=\{1,3\}$, and $\S_3=\{2,3\}$, and 1 task requiring all of 3 data items.
%Suppose that the user sensing capability is single-minded, i.e., each user $i$ either senses all the data items in $\S_i$, or does not sense  any data item.
%Then, the fractional optimal solution is to schedule each user half of the time, i.e., $x_1^*(\S_1) = x_2^*(\S_2) =  x_3^*(\S_3) = 0.5$, and to complete the task all the time, i.e., $z_1^* = 1$. However, such a fractional solution cannot be implemented in practice.}
%To this end, in the next subsection, we will transform the fractional VCG auction to the randomized auction mechanisms (which are implementable) through proper decompositions.
Next, we will transform $\mech^\ast$ to the randomized auction, which always generates a feasible solution to Problem P1 randomly according to certain probability. %, hence is implementable.

%\com{At the end of this paragraph, motivates us our study of the randomized auction design. How does this resolve the implementation issue? What is the corresponding tradeoff (summary at a very high level)? }

%We consider the relaxed problem, where we relax $x_{i}(\S),y_d,z_j\in\{0,1\}$ to be $x_{i}(\S)\geq 0,y_d\geq 0,z_j\geq 0$. This problem becomes the following linear programming problem.
%\begin{align}
%&\max~~\sum_{j\in\J}v_jz_j-\sum_{i\in\I}\sum_{\S\in\B_i}b_i(\S)x_{i}(\S)\label{eq:twosidedalloationproblemRelax}\\
%&~\mathrm{s.t.} ~~~\sum_{\S\in\B_i}x_{i}(\S)\leq1, \text{~~~~~~~~~~~~~$\forall i\in\I$}\label{eq:twosidedcon1Relax}\\
%&~~~~~~~~z_j\leq y_d,~~~~~~~~~~~~~~~~~~~~~~\forall j\in\J,\forall d\in\D_j\label{eq:twosidedcon2Relax}\\
%&~~~~~~~~y_{d}\leq\sum_{i\in\I}\sum_{\S\in\B_i:d\in\S}x_{i}(\S),~~~ \forall d\in\D\label{eq:twosidedcon3Relax}\\
%&~\mathrm{var.}~~x_{i}(\S)\geq 0\text{~~~~~~~~~~~~~~~~$\forall i\in\I,\S\in\B_i$}\\
%&~~~~~~~~y_d\geq 0 \text{~~~~~~~~~~~~~~~~~~~~$\forall d\in\D$}\\
%&~~~~~~~~z_j\geq 0 \text{~~~~~~~~~~~~~~~~~~~~$\forall j\in\J$}.\label{eq:twosidedcon5Relax}
%\end{align}
%The linear programming problem can be optimally solved in polynomial time. We denote the optimal solution to the linear programming problem as $\x ^{\ast}=\{x_i^{\ast}(\S), i\in\I,\S\in\B_i\}$ and $\z ^{\ast}=\{z_j^{\ast}, j\in\J\}$, which specifies which user will be selected with which data bundles and which tasks will be selected in the fractional domain.



%
%\textbf{Truthful Fractional Mechanism:} With the allocation solution $\x ^{\ast}=\{x_i^{\ast}(\S), i\in\I,\S\in\B_i\}$, we can immediately give the fractional VCG prices $\p ^{\ast}=\{p_i^{\ast},i\in\I\}$, i.e.,
%\begin{align}
%p_i^{\ast}&=\max_{\substack{\{z_j\geq 0\}_{j\in\J}\\   \{x_{i'}(\S)\geq 0\}_{i'\neq i}}}\left(\sum_{j\in\J}^{}v_jz_j-\sum_{i'\in\I\setminus\{i\}}\sum_{\S\in\B_{i'}}b_{i'}(\S)x_{i'}(\S)\right)\notag\\
%&~~~-\left(\sum_{j\in\J}^{}v_jz_j^{\ast}-\sum_{i'\neq i,i'\in\I}\sum_{\S\in\B_{i'}}b_{i'}(\S)x^{\ast}_{i'}(\S)\right).
%%\max_{\{\T_j\}_{j\neq m}}\sum_{j\neq m}\max \sum_{m\in\M}\sum_{\S\subseteq\T}(v(\S)-b_m(\S))x_{m}(\S)
%\end{align}
%
%Provide the fractional truthful mechanism (Mechanism 1):
%
%(i) Allocation Mechanism: the fractional optimal solution of the above problem,  $\x^*, \z^*$;
%
%(ii) Payment Mechanism: payment is based on VCG mechanism, $\p^*$.
%
%\begin{proposition}
%The above fractional mechanism is truthful, individual rational, and incentive compatible.
%\end{proposition}
%
%
%\vspace{3cm}


\subsubsection{\textbf{Randomized Mechanism Basics}}\label{sec:ram}

%Key task: Transfer the Fractional Truthful Mechanism to Randomized Truthful Mechanism

%Definition of  randomized mechanism ...

%Definition of truthful in expectation for randomized mechanism ...

%In this section, we will transform the truthful fractional mechanism to the truthful randomized mechanism.

%We first explain what is a randomized mechanism.
%\subsubsection{Randomized Mechanism Basics}
\revl{We first introduce the key concepts in randomized mechanisms \cite{ra}.}
%\com{Are we the first one looking at randomized auction mechanism? If not, which formulation/mechanism/results are related to which key literature? }

Recall that a two-sided \emph{deterministic} mechanism $\mech = \{\x (\cdot), \z (\cdot); \p(\cdot),\pv(\cdot)\}$  consists of a deterministic  allocation rule $\{\x (\cdot), \z (\cdot)\}$ and a payment rule $\{\p (\cdot),\pv(\cdot)\}$, and returns a deterministic  outcome $\{\x (\b,\bv ), \z (\b,\bv ); \p (\b,\bv ),\pv(\b,\bv)\}$ given any bids $\b $ and $\bv$.
Note that both $\mech^o$ and $\mech^*$ mentioned above are deterministic mechanisms.
%Recall that a (direct revelation) mechanism consists of an allocation rule (that is, an algorithm) $\x$, and a pricing scheme $p_i$ for each player.
%Each player $i$ reports a type $b_i$ (possibly deviating from his true type), and the mechanism computes the outcome $\x$ and charges price $p_i$ to player $i$.

A mechanism $\wmech \eq  \{\wx (\cdot), \wz (\cdot); \wp (\cdot),\wpv(\cdot)\}$ can also be randomized, %\footnote{For clarity, we use the tilde ``$\sim$'' to denote a randomized mechanism.}
in which it will flip coins to determine the allocation and payment, instead of giving out a deterministic allocation and payment.
In other words, given any bids $\b $~and~$\bv$, the outcomes $\widetilde{x}_i(\b,\bv )$, $\widetilde{z}_j(\b,\bv  )$, $\widetilde{p}_i(\b,\bv)$ and $\widetilde{q}_j(\b,\bv)$ are all random variables. Moreover, each task's utility (i.e., value minus charge) and each user's utility (i.e., payment minus sensing cost) are also random variables.
Intuitively, such a randomized mechanism can be viewed as a set of randomizations over the deterministic mechanism.
For randomized mechanisms, the concept of truthfulness is defined in the expected sense.
%Formally,
%Formally, we define truthfulness in expectation as follows.
% and in which case $x_i(b)$ and $p_i(b)$ are random variables, and a player's utility is also a random variable. That is, a randomized mechanism is the randomizations over the deterministic mechanism. For randomized mechanisms, truthfulness is in the expected sense. Formally, we define truthfulness in expectation as follows.
% \begin{definition}[Truthfulness in Expectation \cite{ra}]
% A randomized mechanism $\wmech = \{\wx (\cdot), \wz (\cdot); \wp (\cdot),\wpv (\cdot)\}$ is truthful in expectation,
% if and only if (i) for any user $i$, under any other users' bids $\b_{-i}$ and all task bids $\bv$,
% $$
% \mathbb{E}[U_i(\c_i, \b_{-i},\bv) ]
% \geq
% \mathbb{E}[U_i(\b'_i, \b_{-i},\bv) ] , \quad \forall \b'_i \neq \c_i,
% $$
% where $U_i(\b_i, \b_{-i},\bv) = \widetilde{p}_i(\b_i, \b_{-i},\bv) - C_i (\wx(\b_i, \b_{-i},\bv))$ is the user $i$'s utility (random variable) when submitting  the bid $\b_i$; and (ii) for any task $j$, under any other tasks' bids $\bv_{-j}$ and all user bids $\b$,
% $$
% \mathbb{E}[U_j(\v_j, \bv_{-j},\b) ]
% \geq
% \mathbb{E}[U_j(\v'_j, \bv_{-j},\b) ] , \quad \forall \bv'_j \neq \v_j,
% $$
% where $U_j(\bv_j, \bv_{-j},\b) \!=\!  v_j (\wz(\bv_j, \bv_{-j},\b))-\widetilde{\hat{p}}_j(\bv_j, \bv_{-j},\b)$ is the task $j$'s utility (random variable) when submitting  the bid $\bv_j$.
% %and $b_{-i}\in \B_{-i}$, and any $\bar{b}_i,b_i'\in \B_i,$ $\mathbb{E}[\bar{b}_i(x(\bar{b}_i,b_{-i}))-p_i(\bar{b}_i,b_{-i})]\geq \mathbb{E}[\bar{b}_i(x(b_i',b_{-i}))-p_i(b_i',b_{-i})]$.
% \end{definition}
That is, if a randomized mechanism $\wmech$ is truthful in expectation, then the \emph{expected} utilities of each user and each task are maximized when reporting truthfully. %\footnote{\revx{Note that the concept of truthfulness in expectation for randomized mechanisms is as strong as the truthfulness for deterministic mechanisms \cite{ra}.}}
%regardless of what the other users report.

%A randomized algorithm is often viewed as specifying a probability distribution over deterministic algorithms.


\subsubsection{\textbf{Randomized Mechanism Design Criterion}}
We now provide the design criterion of a randomized mechanism.
% : \emph{find a randomized mechanism that generates the equivalent outcome of a truthful deterministic mechanism}.

We first introduce an $(\alpha,\beta)$-scaled fractional mechanism  for the (deterministic) mechanism $ \mech = \{\x (\cdot), \z(\cdot); \p(\cdot),\pv(\cdot) \}$, inspired by the $\alpha$-scaled fractional mechanism defined in \cite{ra,RAuction}. The key difference between the $\alpha$-scaled fractional mechanism in \cite{ra,RAuction} and the $(\alpha,\beta)$-scaled fractional mechanism is that the former one considers only the scaling of one side, while our mechanism considers the scaling of both sides.

\begin{definition} [Scaled Fractional Mechanism]
An $(\alpha,\beta)$-scaled fractional mechanism of $\mech =\{\x (\cdot), \z(\cdot);  \p(\cdot),\pv(\cdot)\}$, denoted by
 $\mech_{(\alpha,\beta)} = \{\x_\alpha(\cdot), \z_\beta(\cdot); \p_\alpha(\cdot),\pv_\beta(\cdot)\}$, is defined as:
\begin{gather}
 \textstyle
\x_\alpha(\cdot)  = {\alpha} \cdot  \x (\cdot),\ \
%  = ( {\alpha }\cdot {x_i} (\cdot) )_{i\in I},
\p_\alpha (\cdot) = {\alpha}  \cdot \p(\cdot),\\
 \z_\beta(\cdot)  = {\beta} \cdot  \z (\cdot), \ \
%  = ( {\alpha }\cdot {x_i} (\cdot) )_{i\in I},
\pv_\beta (\cdot) = {\beta}  \cdot \pv(\cdot),
%  = ( {\alpha } \cdot {p_i} )_{i\in I},
\end{gather}
%and $ \x_\alpha (\cdot) $ is any feasible user scheduling under task selection $  \z_\alpha (\cdot) $, %\footnote{\revv{There may be many $\alpha$-scaled fraction mechanisms $\mech_\alpha$ for a mechanism $\mech$, due to  the multiple choices of $\x_\alpha(\cdot)$.}}
where $ {\alpha},{\beta} > 0$ are the scaling factors with $0 \preceq   {\alpha} \cdot  \x (\cdot) \preceq 1 $ and $0 \preceq   {\beta} \cdot  \z (\cdot) \preceq 1 $, respectively.
 %\com{If $z_\alpha$ is ANY feasible task selection, then there are many $\alpha$-scaled fraction mechanisms starting from the same mechanism $\{x,z;p\}$?}
\end{definition}

Intuitively, in an $ ({\alpha},\beta)$-scaled fractional mechanism, the incurred cost and payment of each user are scaled with~$\alpha$, and the achieved value and charge of each task are scaled with $\beta$, compared with those in the original mechanism~$\mech$. Thus,
% This implies that both the users' and the task owners' optimal bidding strategies in these two mechanisms are equivalent, which leads to the equivalence of their truthfulness. %\footnote{Due to space limit, we put all proofs in the online technical report \cite{TechRpt}.}
%\revv{Note that the user scheduling can be different in these two mechanisms.}
%\revl{Formally, we are able to prove the truthfulness of $\mech_{({\alpha},\beta)}$.}

%\com{Please mention that the completion tasks can be different in these two mechanisms .This avoids giving readers the impressions that both mechanisms are entirely equivalent. }

\begin{proposition}\label{prop:xx1}
If a mechanism $\mech $ is truthful, then its $({\alpha},\beta)$-scaled fractional mechanism
$\mech_{(\alpha,\beta)} $ is also truthful.
\end{proposition}


Based on the above, we propose the following truthful randomized mechanism design criterion:
\begin{itemize}
  \item \emph{Design a randomized mechanism $\wmech$ that generates the equivalent outcome (in terms of the task selection, user scheduling, and payment) as an $({\alpha},\beta)$-scaled fractional mechanism $\mech^*_{({\alpha},\beta)} $ of the fractional VCG auction~$\mech^*$}.
\end{itemize}
\revx{As $\mech^*$ is truthful, we can obtain the truthfulness of its $({\alpha},\beta)$-scaled fractional mechanism $\mech^*_{({\alpha},\beta)} $ by Proposition~\ref{prop:xx1}.
Moreover, as  $\wmech $ generates the same task selection, user scheduling, and payment as $\mech^*_{({\alpha},\beta)} $,
we can further obtain the truthfulness (in expectation) of the randomized mechanism $ \wmech$.
%Namely,
%$$
%\mbox{Truthfulness:}
%\quad \mech^* 	\Rightarrow  \mech^*_\alpha \Rightarrow \wmech.
%$$
}

%\com{This paragraph is not very clear.
%You mention three mechanisms here.
%The second is the $\alpha$-scaled version of the third one.
%What is the connection between the first and second?}


\subsubsection{\textbf{Truthful Randomized Mechanism}}
Now we design the truthful randomized mechanism.

%\com{Why do we use $\lambda$ as both superbscript and subscript? Let us make the position consistent in both notations. }
For convenience, we express a randomized mechanism $
\wmech =  \{\wx(\cdot), \wz(\cdot); \wp (\cdot),\wpv (\cdot)\} $ as a set of allocation probabilities $\boldsymbol{\lambda} = (\lambda^l)_{l\in \A}$ and a set of payment rules $\{\p^l(\cdot), \pv^l(\cdot) \}_{l\in\A}$ under all possible allocations,
 where $\A$ is the set of all feasible \emph{integer} allocations (regarding $ \x $ and $ \z $) and $\lambda^l \geq 0$ is the probability of picking up a particular allocation $\{\x^l, \z^l\}$ and an associated  payment $ \{\p^l, {\pv}^l\}$.
Then, designing a randomized mechanism $\wmech $ is equivalent to finding a set of allocation  probabilities $\boldsymbol{\lambda} = (\lambda^l)_{l\in \A}$ and a set of payment rules $\{ \p^l (\cdot),{\pv}^l(\cdot)\}_{l\in\A}$.


%\com{my overall feeling that our paper is like a math paper without engineering insights in presenting such theoretical mechanisms or key results.
%For example, we only present Prop. 6 and 7 about the satisfaction of the two properties. Most economic mechanisms satisfy these, so what? Where is the engineering insights from the analytical results? }



%\com{This paragraph should be given BEFORE the two mechanisms. }

Next, we propose the randomized auction~$\wmech$, which aims to maximize the
two-sided scaled social welfare subject to the exact decomposition of the fractional optimal solution into the weighted sum of integer solutions.
%on top of the fractional VCG auction $\mech^*$. (i.e., the fractional optimal solution).
Due to the two-sided social welfare maximization, $\wmech$ nontrivially  extends those with one-sided utility maximization or cost minimization in \cite{ra,RAuction}.
%scaled total expected values of tasks minus the scaled total expected sensing costs of users.
%total expected value of tasks, while maintaining the expected sensing cost of each user at the level of the fractional VCG auction $\mech^*$ (i.e., the fractional optimal solution).
%The randomized mechanism $\wmech^\ddag$ aims to minimize the expected sensing cost of each user (with the same scaling factor $\alpha$ for all users),
%while maintaining the total expected value of all tasks at the level of the fractional VCG auction $\mech^*$.

%\setcounter{mechanism}{2}
\begin{mechanism}[Randomized Auction Mechanism -- $\wmech$]\label{mech:3}~

%\revx{Starting from the fractional VCG auction $\mech^* = \{\x^\ast(\b,\bv) ,$ $\z^\ast(\b,\bv); \p^\ast(\b,\bv),{\pv}^\ast(\b,\bv)\}$, we define the randomized auction mechanism $\wmech$ as:}
\begin{itemize}
\item
%\com{It is not clear what is the starting point of this randomized mechanism. In particular, do we start with a particular fractional mechanism (what is the notation) and do proper scaling? Or we are looking at all feasible integer solutions?
%\\
%In other words, we need to explain clearly all the notations used in this mechanism within the mechanism.}
Allocation Rule  $\boldsymbol{\widetilde{\lambda}} = (\lambda^l)_{l\in \A}$:
\begin{equation*}
\begin{aligned}
\textstyle \boldsymbol{\widetilde{\lambda}}  =  &  \arg \max_{\boldsymbol{\lambda}, 0<\alpha,\beta\leq 1} ~~ \beta\cdot V^\ast-\alpha\cdot C^\ast
\\
& \textstyle \mbox{s.t.,}\textstyle  \sum_{l \in \A}
\lambda^l \cdot
\x_i^l = \alpha  \cdot\x_i^\ast (\b,\bv) , \quad \forall i\in \I,\\
& ~~~~\textstyle \sum_{l \in \A}
\lambda^l \cdot
z_j^l  = \beta  \cdot  z_j^\ast (\b,\bv), \quad \forall j\in \J,
\end{aligned}
\end{equation*}
where $V^\ast$ and $C^{\ast}$ are the optimal total task values and user costs w.r.t. $\z^\ast(\b,\bv)$ and $\x^\ast(\b,\bv)$, respectively.
\item
Payment Rule  $\{\p^l (\b,\bv),{\pv}^l(\b,\bv) \}_{l\in \A} $:
\begin{gather}
\textstyle
p_i^{l} (\b,\bv) = \alpha \cdot p_i^\ast (\b,\bv) \cdot \frac{C_i(\x_i^l)}{ \sum_{l' \in \A}
\lambda_{l'} \cdot
C_i(\x_i^{l'}) },\forall i\in\I,\notag\\
\textstyle
{q}_j^{l} (\b,\bv) = \beta \cdot q_j^\ast (\b,\bv) \cdot \frac{V_j(z_j^l)}{ \sum_{l' \in \A}
	\lambda_{l'} \cdot
	V_j(z_j^{l'}) },\forall j\in\J,\notag
\end{gather}
where $C_i(\x_i^l)$ is user $i$'s cost under the allocation $\x_i^l$, and $V_j(z_j^l)$ is task $j$'s value under the allocation $z_j^l$.
\end{itemize}
\end{mechanism}



% \begin{mechanism}[Randomized Auction Mechanism -- $\wmech^\ddag$]\label{mech:4}
% ~

% \revx{Starting from the fractional VCG auction $\mech^* = \{\x^\ast(\cdot) ,$ $\z^\ast(\cdot); \p^\ast(\cdot)\}$, we define the randomized mechanism $\wmech^\ddag$ as:}
% \begin{itemize}
% \item
% %\com{Same comment as Mechanism 3. }
% Allocation Rule  $\boldsymbol{\lambda} = (\lambda^l)_{l\in \A}$:
% \begin{equation*}
% \begin{aligned}
% \boldsymbol{\lambda}  =  &  \arg \min_{\boldsymbol{\lambda}, \gamma\geq 1} ~~ \gamma
% \\
% & \mbox{s.t.,}\sum_{j\in \J}  \sum_{l \in \A}
% \lambda^l \cdot
% z_j^l \cdot v_j =\sum_{j\in \J}  z_j^\ast (\b) \cdot v_j  ;
% \\
% & ~~~~  \sum_{l \in \A}
% \lambda^l \cdot
% \x_i^l = \gamma \cdot \x_i^\ast (\b) , \quad \forall i\in \I.
% \end{aligned}
% \end{equation*}
% \item
% Payment Rule  $(\p^l (\b))_{l\in \A}$:
% $$
% p_i^{l}(\b) = \gamma \cdot p_i^\ast(\b) \cdot \frac{C_i(\x_i^l)}{ \sum_{l' \in \A}
% \lambda_{l'} \cdot
% C_i(\x_i^{l'}) },
% $$
% where $C_i(\x_i^l)$ is the user $i$'s cost under allocation $\x_i^l$.
% \end{itemize}
% \end{mechanism}

Obviously, both the expected payment and sensing cost of each user  \emph{and} the expected charge and value of each task in $\wmech$ are equivalent to those in  $\mech^*_{({\alpha},\beta)} $, which implies that $\wmech$ is truthful (incentive compatible) \emph{in expectation}, in the sense that each user and task can maximize their expected utilities when reporting truthfully. Formally, %; in mechanism $\wmech^\ddag$, the expected payment and sensing cost of each user are equivalent to those in an $\alpha$-scaled fractional auction  of $\mech^*$,
%which also implies that $\wmech^\ddag$ is truthful \emph{in expectation}.
%Formally, we have the following proposition.


%Rewrite a randomized mechanism $\{\x^\dag, \p^\dag\}$ as a set of probabilities  $\boldsymbol{\lambda} = (\lambda^l)_{l\in A}$, where $\lambda^l \geq 0$ and $\sum_{l\in A} \lambda^l = 1$.
%
%In this section, we want to find such a set of probabilities $\boldsymbol{\lambda} = (\lambda^l)_{l\in A}$ that achieves the fractional optimal data value and meanwhile minimizes the expected sensing cost. Namely,
%$$
%\sum_{l \in A} \lambda^l \cdot \z_l(j) = z_j^* , \quad \forall j\in J ;
%$$
%$$
%\sum_{i \in I} \sum_{l \in A} \lambda^l \cdot \x_l(i) \cdot c_j (\x_l) \mbox{~~is minimized.}
%$$
%
%\vspace{3cm}
%
%\subsubsection{Randomized Truthful Mechanism B}
%
%
%In this section, we want to find such a set of probabilities $\boldsymbol{\lambda} = (\lambda^l)_{l\in A}$ that maximizes the expected data value and meanwhile guarantees the fractional optimal sensing cost. Namely,
%$$
%\sum_{l \in A} \lambda^l \cdot \x_l(i) = x_i^* , \quad \forall i\in I;
%$$
%$$
%\sum_{j \in I} \sum_{l \in A} \lambda^l \cdot \z_l(j) \cdot v_j (\z_l) \mbox{~~is maximized.}
%$$
%


%\subsection{Randomized Mechanism}
%The set $\{\lambda^l,l\in\I\}$ can be viewed as a probability distribution over the integer solutions $\x ^l,l\in\I$. The randomized mechanism is given as follows.
%
%\textbf{Allocation:} select each integer solution $\x ^l$ with the probability $\lambda^l$; and then output the allocation $(\S_1^l,\cdots,\S_I^l)$ defined by $\x ^l$.
%
%\textbf{Payment:} for each winner $n$ such that ${x}_i^l=1$, the price is
%$$p_i^{l}=p_i^{\ast}\cdot \frac{b_i(\S_i^l)}{b_i(\x ^{\ast})}.$$
%
%\subsection{Analysis}
%Let $X_i(\S)$ be a binary random variable that takes value 1 iff $\S_i=\S$. Then the payment to bidder $i$ is
%$$
%P_i=\sum_{\S\in\B_i}\frac{b_i(\S)X_i(\S)}{b_i(\x ^{\ast})}p_i^{\ast}.
%$$

%\com{How to prove Propositions 6 and 7? }

\begin{proposition}
The randomized mechanisms $\wmech$ is incentive compatible (truthful) in expectation.
\end{proposition}


We can further check that under the mechanism $\wmech$, each user and task can always achieve a non-negative utility \emph{under any possible realization of allocations}. This implies that
 $\wmech$ is individually rational \emph{in the strict sense}. Formally,

\begin{proposition}
The randomized mechanisms $\wmech$ is individually rational in the strict sense.
\end{proposition}



\revx{Furthermore, we can see that in $\wmech$, each user's sensing cost equals $\alpha^*$ times the sensing cost incurred in $\mech^*$, while each task's value equals $\beta^*$ times the value achieved in $\mech^*$ (where $\alpha^*,\beta^*$ are the optimal solutions to the allocation problem in $\wmech$).
%Similarly, in mechanism $\wmech^\ddag$, the total achieved task value equals that in $\mech^*$, while the sensing cost of each user equals $\gamma^*$ times its sensing cost in $\mech^*$ (where $\gamma^*$ is the   solution to the allocation problem in $\wmech^\ddag$ ).
Hence,   the efficiency of     $\wmech$ is guaranteed in this sense.}~~~~~

\begin{proposition}[Efficiency of $\wmech$]
The mechanism $\wmech$ guarantees to achieve a $\beta^*$-fraction of the total task values in $\mech^*$ with an $\alpha^*$-fraction of the total sensing costs in $\mech^*$.
\end{proposition}
% \begin{proposition}[Efficiency of Mechanism $\wmech^\ddag$]
% The mechanism $\wmech^\ddag$ guarantees to achieve the same total task value in $\mech^*$ with a $\gamma^*$-times of the sensing cost in $\mech^*$.
% \end{proposition}}

%\revv{\begin{proposition}[Efficiency (Conditioned)]
%Mechanism A guarantees to achieve a $\beta^*$-times of the fractional optimal task value, given the sensing costs of users in the fractional optimal solution,
%and Mechanism B guarantees to achieve an $\alpha^*$-times of the fractional optimal sensing cost, given the total value of all tasks in fractional optimal solution,
%where $\beta^*$ and  $\alpha^*$ are the optimal solutions of allocation problems in mechanisms A and B, respectively.
%\end{proposition}}



%\com{Should these two results be stated as official propositions? }

%\begin{lemma}[Individual Rationality]
%The randomized mechanism satisfies the Individual Rationality property, i.e.,
%$$
%U_i(c_i,b_{-i})\geq 0.
%$$
%\end{lemma}
%\begin{IEEEproof}
%Suppose the realization of the randomized mechanism is $(\x ^l,\p ^l)$, by truth telling, the utility of user $n$ is
%$$
%U_i(c_i,b_{-i})=p_i^l-c_i(\S_i^l)=\frac{c_i(\S_i^l)}{c_i(\x ^{\ast})}p_i^{\ast}-c_i(\S_i^l)\geq0,
%$$
%due to the Individual Rationality of VCG mechanisms, i.e., $p_i^{\ast}-c_i(\x ^{\ast})\geq0$.
%\end{IEEEproof}
%
%\begin{lemma}[Incentive Compatibility in Expectation]
%The randomized mechanism satisfies the Incentive Compatibility property in the expected sense.
%\end{lemma}
%\begin{IEEEproof}
%We note that $\mathbb{E}[X_i(\S)]=\mathrm{Pr}[\S_i=\S]=\sum_l\lambda^lx_{i}^l(\S)=x_i^{\ast}(\S)$, and
%\begin{align}
%\mathbb{E}[P_i]&=\mathbb{E}\left[\sum_{\S\in\B_i}\frac{b_i(\S)X_i(\S)}{b_i(\x ^{\ast})}p_i^{\ast}\right]\notag\\
%&=\sum_{\S\in\B_i}\frac{b_i(\S)\mathbb{E}[X_i(\S)]}{b_i(\x ^{\ast})}p_i^{\ast}\notag\\
%&=\sum_{\S\in\B_i}\frac{b_i(\S)\frac{x_i^{\ast}(\S)}{\alpha_i}}{b_i(\x ^{\ast})}p_i^{\ast}\notag\\
%&=p_i^{\ast}.
%\end{align}
%
%Since the utility of user $i$ is $U_i(b)=P_i-\sum_{\S\in\B_i}b_i(\S)X_i(\S)$, we have
%\begin{align}
%\mathbb{E}[U_i(b)]&=\mathbb{E}\left[P_i-\sum_{\S\in\B_i}b_i(\S)X_i(\S)\right]\notag\\
%&=\mathbb{E}[P_i]-\sum_{\S\in\B_i}b_i(\S)\mathbb{E}[X_i(\S)]\notag\\
%&=p_i^{\ast}-\sum_{\S\in\B_i}b_i(\S)x_i^{\ast}(\S)\notag\\
%&=u_i(b).
%\end{align}
%Hence, the Incentive Compatibility follows from the Incentive Compatibility of the deterministic VCG mechanisms.
%\end{IEEEproof}

%\begin{lemma}[Social Efficiency]
%The randomized mechanism achieves an $\boldsymbol{\alpha}$ approximation ratio to the fractional optimal social welfare.
%\end{lemma}
%\begin{IEEEproof}
%The expected sensing cost is
%$$
%\begin{aligned}
%\mathbb{E}\left[\sum_{i\in\I}b_i(\S_i^l)\right]&=\mathbb{E}\left[\sum_i\sum_{\S\in\B_i}b_i(\S)X_i(\S)\right]\\
%&=\sum_{i\in\I}\sum_{\S\in\B_i}b_i(\S)\mathbb{E}[X_i(\S)]\\
%&=\sum_{i\in\I}\sum_{\S\in\B_i}b_i(\S)x_i^{\ast}(\S).
%\end{aligned}
%$$

%The expected social welfare depends on the task value terms...
%\end{IEEEproof}
%
%\begin{lemma}[Truthfulness in Expectation]
%The randomized mechanisms $A$ and $B$ are truthful in expectation.
%\end{lemma}
%
%\begin{theorem}
%The Randomized Mechanism is truthful in expectation and achieves a $\boldsymbol{\alpha}$-approximation to the optimal social welfare with polynomial-time complexity. Besides, it satisfies the Individual Rationality and Incentive Compatibility in Expectation.
%\end{theorem}



